MLQD: A package for machine learning-based quantum dissipative dynamics

Machine learning has emerged as a promising paradigm to study the quantum dissipative dynamics of open quantum systems. To facilitate the use of our recently published ML-based approaches for quantum dissipative dynamics, here we present an open-source Python package MLQD (https://github.com/Arif-PhyChem/MLQD), which currently supports the three ML-based quantum dynamics approaches: (1) the recursive dynamics with kernel ridge regression (KRR) method, (2) the non-recursive artificial-intelligence-based quantum dynamics (AIQD) approach and (3) the blazingly fast one-shot trajectory learning (OSTL) approach, where both AIQD and OSTL use the convolutional neural networks (CNN). This paper describes the features of the MLQD package, the technical details, optimization of hyperparameters, visualization of results, and the demonstration of the MLQD's applicability for two widely studied systems, namely the spin-boson model and the Fenna--Matthews--Olson (FMO) complex. To make MLQD more user-friendly and accessible, we have made it available on the XACS cloud computing platform (https://XACScloud.com) via the interface to the MLatom package (http://MLatom.com).

==> main <==
@PREAMBLE{
 "\providecommand{\noopsort}[1]{}" 
 # "\providecommand{\singleletter}[1]{#1}%" 
}
@article{rodriguez2022comparative,
  title={A comparative study of different machine learning methods for dissipative quantum dynamics},
  author={Rodr{\'\i}guez, Luis E Herrera and Ullah, Arif and Espinosa, Kennet J Rueda and Dral, Pavlo O and Kananenka, Alexei A},
  journal={Machine Learning: Science and Technology},
  volume={3},
  number={4},
  pages={045016},
  year={2022},
  publisher={IOP Publishing}
}
@article{ullah2021speeding, 
year = {2021}, 
keywords = {ML QD Collaboration with Dral and Lan}, 
title = {{Speeding up quantum dissipative dynamics of open systems with kernel methods}}, 
author = {Ullah, Arif and Dral, Pavlo O}, 
journal = {New Journal of Physics} 
}
@article{han2020stochastic,
  title={Stochastic equation of motion approach to fermionic dissipative dynamics. I. Formalism},
  author={Han, Lu and Ullah, Arif and Yan, Yun-An and Zheng, Xiao and Yan, YiJing and Chernyak, Vladimir},
  journal={The Journal of Chemical Physics},
  volume={152},
  number={20},
  pages={204105},
  year={2020},
  publisher={AIP Publishing LLC}
}
@article{ullah2020stochastic,
  title={Stochastic equation of motion approach to fermionic dissipative dynamics. II. Numerical implementation},
  author={Ullah, Arif and Han, Lu and Yan, Yun-An and Zheng, Xiao and Yan, YiJing and Chernyak, Vladimir},
  journal={The Journal of Chemical Physics},
  volume={152},
  number={20},
  pages={204106},
  year={2020},
  publisher={AIP Publishing LLC}
}

@article{lin2022trajectory,
  title={Trajectory Propagation of Symmetrical Quasi-classical Dynamics with Meyer-Miller Mapping Hamiltonian Using Machine Learning},
  author={Lin, Kunni and Peng, Jiawei and Xu, Chao and Gu, Feng Long and Lan, Zhenggang},
  journal={The Journal of Physical Chemistry Letters},
  volume={13},
  pages={11678--11688},
  year={2022},
  publisher={ACS Publications}
}
@article{ullah2023qd3set,
  title={QD3SET-1: A Database with Quantum Dissipative Dynamics Data Sets},
  author={Ullah, Arif and Rodr{\'\i}guez, Luis E Herrera and Dral, Pavlo O and Kananenka, Alexei A},
  journal={Frontiers in Physics},
  volume={11},
  pages={1223973},
  year={2023},
  publisher={Frontiers}
}
@article{lin2022automatic,
  title={Automatic Evolution of Machine-Learning based Quantum Dynamics with Uncertainty Analysis},
  author={Lin, Kunni and Peng, Jiawei and Xu, Chao and Gu, Feng Long and Lan, Zhenggang},
  journal={arXiv preprint arXiv:2205.03600},
  year={2022}
}
@article{ullah2022predicting,
  title={Predicting the future of excitation energy transfer in light-harvesting complex with artificial intelligence-based quantum dynamics},
  author={Ullah, Arif and Dral, Pavlo O},
  journal={Nature communications},
  volume={13},
  number={1930},
  pages={1--8},
  year={2022},
  publisher={Nature Publishing Group}
}
@article{dral2019mlatom,
  title={MLatom: A program package for quantum chemical research assisted by machine learning},
  author={Dral, Pavlo O},
  journal={Journal of computational chemistry},
  volume={40},
  number={26},
  pages={2339--2347},
  year={2019},
  publisher={Wiley Online Library}
}
@article{herrera2021convolutional,
  title={Convolutional neural networks for long time dissipative quantum dynamics},
  author={Herrera Rodríguez, Luis E and Kananenka, Alexei A},
  journal={The Journal of Physical Chemistry Letters},
  volume={12},
  number={9},
  pages={2476--2483},
  year={2021},
  publisher={ACS Publications}
}
@article{ullah2022one,
  title={One-Shot Trajectory Learning of Open Quantum Systems Dynamics},
  author={Ullah, Arif and Dral, Pavlo O.},
  journal={The Journal of Physical Chemistry Letters},
  volume={13},
  number={26},
  pages={6037--6041},
  year={2022},
  publisher={ACS Publications}
}
@Inbook{rasmussen2003gaussian,
author={Rasmussen, Carl Edward},
title={Gaussian Processes in Machine Learning},
bookTitle={Advanced Lectures on Machine Learning: ML Summer Schools 2003, Canberra, Australia, February 2 - 14, 2003, T{\"u}bingen, Germany, August 4 - 16, 2003, Revised Lectures},
year={2004},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={63--71}
}

@article{gneiting2010matern,
  title={Mat{\'e}rn cross-covariance functions for multivariate random fields},
  author={Gneiting, Tilmann and Kleiber, William and Schlather, Martin},
  journal={Journal of the American Statistical Association},
  volume={105},
  number={491},
  pages={1167--1177},
  year={2010},
  publisher={Taylor \& Francis}
}
@article{dral2021mlatom,
  title={MLatom 2: An Integrative Platform for Atomistic Machine Learning},
  author={Dral, Pavlo O and Ge, Fuchun and Xue, Bao-Xin and Hou, Yi-Fan and Pinheiro, Max and Huang, Jianxing and Barbatti, Mario},
  journal={Topics in Current Chemistry},
  volume={379},
  number={4},
  pages={1--41},
  year={2021},
  publisher={Springer}
}
@Manual{MLatomdev,
  Title                    = {\textit{MLatom}: a Package for Atomistic Simulations with Machine Learning. \href{http://mlatom.com}{http://mlatom.com} (accessed on Feb 13, 2023)},
  Address                  = {Xiamen, China},
  Author                   = {Pavlo O. Dral and Peikun Zheng and Bao-Xin Xue and Fuchun Ge and Yi-Fan Hou and Max Pinheiro, Jr and Yuming Su and Yiheng Dai and Yangtao Chen},
  Organization             = {Xiamen University},
  Year                     = {2013--2023},
  HowPublished             = {Xiamen University, Xiamen, China},
  Institution              = {Xiamen University},
  Publisher                = {Xiamen University}
}
@incollection{dral2020quantum,
  title={Quantum chemistry assisted by machine learning},
  author={Dral, Pavlo O},
  booktitle={Advances in Quantum Chemistry},
  volume={81},
  pages={291--324},
  year={2020},
  editor={Ruud, K. and Br\"{a}ndas, E. J.},
  publisher={Elsevier}
}
@article{stulp2015many,
  title={Many regression algorithms, one unified model: A review},
  author={Stulp, Freek and Sigaud, Olivier},
  journal={Neural Networks},
  volume={69},
  pages={60--79},
  year={2015},
  publisher={Elsevier}
}
@article{caldeira1983path,
  title={Path integral approach to quantum Brownian motion},
  author={Caldeira, Amir O and Leggett, Anthony J},
  journal={Physica A: Statistical mechanics and its Applications},
  volume={121},
  number={3},
  pages={587--616},
  year={1983},
  publisher={Elsevier}
}
@article{ishizaki2009unified,
  title={Unified treatment of quantum coherent and incoherent hopping dynamics in electronic energy transfer: Reduced hierarchy equation approach},
  author={Ishizaki, Akihito and Fleming, Graham R},
  journal={The Journal of chemical physics},
  volume={130},
  number={23},
  pages={234111},
  year={2009},
  publisher={American Institute of Physics}
}
@article{johansson2012qutip,
  title={QuTiP: An open-source Python framework for the dynamics of open quantum systems},
  author={Johansson, J Robert and Nation, Paul D and Nori, Franco},
  journal={Computer Physics Communications},
  volume={183},
  number={8},
  pages={1760--1772},
  year={2012},
  publisher={Elsevier}
}
@article{schmidt2011eighth,
  title={The eighth bacteriochlorophyll completes the excitation energy funnel in the FMO protein},
  author={Schmidt am Busch, Marcel and Muh, Frank and El-Amine Madjet, Mohamed and Renger, Thomas},
  journal={The journal of physical chemistry letters},
  volume={2},
  number={2},
  pages={93--98},
  year={2011},
  publisher={ACS Publications}
}
@article{olbrich2011atomistic,
  title={From atomistic modeling to excitation transfer and two-dimensional spectra of the FMO light-harvesting complex},
  author={Olbrich, Carsten and Jansen, Thomas LC and Liebers, J{\"{o}}rg and Aghtar, Mortaza and Str{\"{u}}mpfer, Johan and Schulten, Klaus and Knoester, Jasper and Kleinekath{\"{o}}fer, Ulrich},
  journal={The Journal of Physical Chemistry B},
  volume={115},
  number={26},
  pages={8609--8621},
  year={2011},
  publisher={ACS Publications}
}
@misc{joseph2019quant,
  author = {Joseph W. Abbott},
  title = {jwa7/quantum{\_}HEOM},
  year = {2019},
  publisher = {GitHub},
  journal = {GitHub repository},
  howpublished = {Github repository: \url{https://github.com/jwa7/quantum_HEOM}, (accessed on Feb 13, 2023)},
}
@article{bourne2019structure,
  title={Structure and efficiency in bacterial photosynthetic light harvesting},
  author={Bourne Worster, Susannah and Stross, Clement and Vaughan, Felix MWC and Linden, Noah and Manby, Frederick R},
  journal={The Journal of Physical Chemistry Letters},
  volume={10},
  number={23},
  pages={7383--7390},
  year={2019},
  publisher={ACS Publications}
}
@misc{joseph2020thesis,
  author = {Joseph W. Abbott},
  title = {Quantum Dynamics of Bath Influenced Excitonic Energy Transfer in Photosynthetic Pigment-Protein Complexes},
  year = {2020},
  journal = {Master Thesis, University of Bristol},
  howpublished = {Master Thesis, University of Bristol United Kingdom \url{https://doi.org/10.5281/zenodo.7229807}}
}
@article{slocombe2022open,
  title={An open quantum systems approach to proton tunnelling in DNA},
  author={Slocombe, Louie and Sacchi, Marco and Al-Khalili, Jim},
  journal={Communications Physics},
  volume={5},
  number={1},
  pages={109},
  year={2022},
  publisher={Nature Publishing Group UK London}
}
@article{dorfman2013photosynthetic,
  title={Photosynthetic reaction center as a quantum heat engine},
  author={Dorfman, Konstantin E and Voronine, Dmitri V and Mukamel, Shaul and Scully, Marlan O},
  journal={Proceedings of the National Academy of Sciences},
  volume={110},
  number={8},
  pages={2746--2751},
  year={2013},
  publisher={National Acad Sciences}
}
@article{rebentrost2009environment,
  title={Environment-assisted quantum transport},
  author={Rebentrost, Patrick and Mohseni, Masoud and Kassal, Ivan and Lloyd, Seth and Aspuru-Guzik, Al{\'a}n},
  journal={New Journal of Physics},
  volume={11},
  number={3},
  pages={033003},
  year={2009},
  publisher={IOP Publishing}
}
@article{plenio2008dephasing,
  title={Dephasing-assisted transport: quantum networks and biomolecules},
  author={Plenio, Martin B and Huelga, Susana F},
  journal={New Journal of Physics},
  volume={10},
  number={11},
  pages={113019},
  year={2008},
  publisher={IOP Publishing}
}
@article{verstraete2009quantum,
  title={Quantum computation and quantum-state engineering driven by dissipation},
  author={Verstraete, Frank and Wolf, Michael M and Ignacio Cirac, J},
  journal={Nature physics},
  volume={5},
  number={9},
  pages={633--636},
  year={2009},
  publisher={Nature Publishing Group UK London}
}
@article{unruh1995maintaining,
  title={Maintaining coherence in quantum computers},
  author={Unruh, William G},
  journal={Physical Review A},
  volume={51},
  number={2},
  pages={992},
  year={1995},
  publisher={APS}
}
@article{yao2021open,
  title={Open quantum systems for quarkonia},
  author={Yao, Xiaojun},
  journal={International Journal of Modern Physics A},
  volume={36},
  number={20},
  pages={2130010},
  year={2021},
  publisher={World Scientific}
}
@book{carmichael2009open,
  title={An open systems approach to quantum optics: lectures presented at the Universit{\'e} Libre de Bruxelles, October 28 to November 4, 1991},
  author={Carmichael, Howard},
  volume={18},
  year={2009},
  publisher={Springer Science \& Business Media}
}
@book{may2008charge,
  title={Charge and energy transfer dynamics in molecular systems},
  author={May, Volkhard and K{\"u}hn, Oliver},
  year={2008},
  publisher={John Wiley \& Sons}
}
@article{sieberer2016keldysh,
  title={Keldysh field theory for driven open quantum systems},
  author={Sieberer, Lukas M and Buchhold, Michael and Diehl, Sebastian},
  journal={Reports on Progress in Physics},
  volume={79},
  number={9},
  pages={096001},
  year={2016},
  publisher={IOP Publishing}
}
@article{wang2022quantum,
  title={Quantum mechanics of open systems: Dissipaton theories},
  author={Wang, Yao and Yan, YiJing},
  journal={The Journal of Chemical Physics},
  volume={157},
  number={17},
  pages={170901},
  year={2022},
  publisher={AIP Publishing LLC}
}
@article{jain2022pedagogical,
  title={Pedagogical Overview of the Fewest Switches Surface Hopping Method},
  author={Jain, Amber and Sindhu, Aarti},
  journal={ACS omega},
  year={2022},
  publisher={ACS Publications}
}
@article{meyer1979classical,
  title={A classical analog for electronic degrees of freedom in nonadiabatic collision processes},
  author={Meyer, Hans-Dieter and Miller, William H},
  journal={The Journal of Chemical Physics},
  volume={70},
  number={7},
  pages={3214--3223},
  year={1979},
  publisher={American Institute of Physics}
}
@article{redfield1957theory,
  title={On the theory of relaxation processes},
  author={Redfield, Alfred G},
  journal={IBM Journal of Research and Development},
  volume={1},
  number={1},
  pages={19--31},
  year={1957},
  publisher={IBM}
}
@article{nakajima1958quantum,
  title={On quantum theory of transport phenomena: steady diffusion},
  author={Nakajima, Sadao},
  journal={Progress of Theoretical Physics},
  volume={20},
  number={6},
  pages={948--959},
  year={1958},
  publisher={Oxford University Press}
}
@article{zwanzig1960ensemble,
  title={Ensemble method in the theory of irreversibility},
  author={Zwanzig, Robert},
  journal={The Journal of Chemical Physics},
  volume={33},
  number={5},
  pages={1338--1341},
  year={1960},
  publisher={American Institute of Physics}
}
@article{xu2018convergence,
  title={Convergence of high order memory kernels in the Nakajima-Zwanzig generalized master equation and rate constants: Case study of the spin-boson model},
  author={Xu, Meng and Yan, Yaming and Liu, Yanying and Shi, Qiang},
  journal={The Journal of chemical physics},
  volume={148},
  number={16},
  pages={164101},
  year={2018},
  publisher={AIP Publishing LLC}
}
@article{silbey1984variational,
  title={Variational calculation of the dynamics of a two level system interacting with a bath},
  author={Silbey, Robert and Harris, Robert A},
  journal={The Journal of chemical physics},
  volume={80},
  number={6},
  pages={2615--2617},
  year={1984},
  publisher={American Institute of Physics}
}
@article{leggett1987dynamics,
  title={Dynamics of the dissipative two-state system},
  author={Leggett, Anthony J and Chakravarty, SDAFMGA and Dorsey, Alan T and Fisher, Matthew PA and Garg, Anupam and Zwerger, Wilhelm},
  journal={Reviews of Modern Physics},
  volume={59},
  number={1},
  pages={1},
  year={1987},
  publisher={APS}
}
@article{cerrillo2014non,
  title={Non-Markovian dynamical maps: numerical processing of open quantum trajectories},
  author={Cerrillo, Javier and Cao, Jianshu},
  journal={Physical review letters},
  volume={112},
  number={11},
  pages={110401},
  year={2014},
  publisher={APS}
}
@book{meyer2009multidimensional,
  title={Multidimensional quantum dynamics: MCTDH theory and applications},
  author={Meyer, Hans-Dieter and Gatti, Fabien and Worth, Graham A},
  year={2009},
  publisher={John Wiley \& Sons}
}
@article{cohen2011memory,
  title={Memory effects in nonequilibrium quantum impurity models},
  author={Cohen, Guy and Rabani, Eran},
  journal={Physical Review B},
  volume={84},
  number={7},
  pages={075150},
  year={2011},
  publisher={APS}
}
@article{beck2000multiconfiguration,
  title={The multiconfiguration time-dependent Hartree (MCTDH) method: a highly efficient algorithm for propagating wavepackets},
  author={Beck, Michael H and J{\"a}ckle, Andreas and Worth, Graham A and Meyer, H-D},
  journal={Physics reports},
  volume={324},
  number={1},
  pages={1--105},
  year={2000},
  publisher={Elsevier}
}
@article{schiro2009real,
  title={Real-time diagrammatic Monte Carlo for nonequilibrium quantum transport},
  author={Schir{\'o}, Marco and Fabrizio, Michele},
  journal={Physical Review B},
  volume={79},
  number={15},
  pages={153302},
  year={2009},
  publisher={APS}
}
@article{anders2005real,
  title={Real-time dynamics in quantum-impurity systems: A time-dependent numerical renormalization-group approach},
  author={Anders, Frithjof B and Schiller, Avraham},
  journal={Physical review letters},
  volume={95},
  number={19},
  pages={196801},
  year={2005},
  publisher={APS}
}
@article{schollwock2005density,
  title={The density-matrix renormalization group},
  author={Schollw{\"o}ck, Ulrich},
  journal={Reviews of modern physics},
  volume={77},
  number={1},
  pages={259},
  year={2005},
  publisher={APS}
}
@article{kananenka2016accurate,
  title={Accurate long-time mixed quantum-classical Liouville dynamics via the transfer tensor method},
  author={Kananenka, Alexei A and Hsieh, Chang-Yu and Cao, Jianshu and Geva, Eitan},
  journal={The journal of physical chemistry letters},
  volume={7},
  number={23},
  pages={4809--4814},
  year={2016},
  publisher={ACS Publications}
}
@article{bergmann2021green,
  title={A Green’s function perspective on the nonequilibrium thermodynamics of open quantum systems strongly coupled to baths: Nonequilibrium quantum thermodynamics},
  author={Bergmann, Nicolas and Galperin, Michael},
  journal={The European Physical Journal Special Topics},
  volume={230},
  pages={859--866},
  year={2021},
  publisher={Springer}
}
@article{anto2021capturing,
  title={Capturing non-Markovian dynamics with the reaction coordinate method},
  author={Anto-Sztrikacs, Nicholas and Segal, Dvira},
  journal={Physical Review A},
  volume={104},
  number={5},
  pages={052617},
  year={2021},
  publisher={APS}
}
@article{nazir2018reaction,
  title={The reaction coordinate mapping in quantum thermodynamics},
  author={Nazir, Ahsan and Schaller, Gernot},
  journal={Thermodynamics in the Quantum Regime: Fundamental Aspects and New Directions},
  pages={551--577},
  year={2018},
  publisher={Springer}
}
@article{xu2016non,
  title={Non-canonical distribution and non-equilibrium transport beyond weak system-bath coupling regime: A polaron transformation approach},
  author={Xu, Dazhi and Cao, Jianshu},
  journal={Frontiers of Physics},
  volume={11},
  pages={1--17},
  year={2016},
  publisher={Springer}
}
@article{cygorek2021numerically,
  title={Numerically exact open quantum systems simulations for arbitrary environments using automated compression of environments},
  author={Cygorek, Moritz and Cosacchi, Michael and Vagov, Alexei and Axt, Vollrath Martin and Lovett, Brendon W and Keeling, Jonathan and Gauger, Erik M},
  journal={arXiv preprint arXiv:2101.01653},
  year={2021}
}
@article{garraway1997nonperturbative,
  title={Nonperturbative decay of an atomic system in a cavity},
  author={Garraway, BM},
  journal={Physical Review A},
  volume={55},
  number={3},
  pages={2290},
  year={1997},
  publisher={APS}
}
@article{luo2023quantum,
  title={A quantum-classical decomposition of Gaussian quantum environments: a stochastic pseudomode model},
  author={Luo, Si and Lambert, Neill and Cirio, Mauro},
  journal={arXiv preprint arXiv:2301.07554},
  year={2023}
}
@article{makarov1994path,
  title={Path integrals for dissipative systems by tensor multiplication. Condensed phase quantum dynamics for arbitrarily long time},
  author={Makarov, Dmitrii E and Makri, Nancy},
  journal={Chemical physics letters},
  volume={221},
  number={5-6},
  pages={482--491},
  year={1994},
  publisher={Elsevier}
}
@article{makri1995numerical,
  title={Numerical path integral techniques for long time dynamics of quantum dissipative systems},
  author={Makri, Nancy},
  journal={Journal of Mathematical Physics},
  volume={36},
  number={5},
  pages={2430--2457},
  year={1995},
  publisher={American Institute of Physics}
}
@article{chin2010exact,
  title={Exact mapping between system-reservoir quantum models and semi-infinite discrete chains using orthogonal polynomials},
  author={Chin, Alex W and Rivas, {\'A}ngel and Huelga, Susana F and Plenio, Martin B},
  journal={Journal of Mathematical Physics},
  volume={51},
  number={9},
  pages={092109},
  year={2010},
  publisher={American Institute of Physics}
}
@article{prior2010efficient,
  title={Efficient simulation of strong system-environment interactions},
  author={Prior, Javier and Chin, Alex W and Huelga, Susana F and Plenio, Martin B},
  journal={Physical review letters},
  volume={105},
  number={5},
  pages={050404},
  year={2010},
  publisher={APS}
}
@article{zhou2018variational,
  title={Variational Study of the Two-Impurity Spin--Boson Model with a Common Ohmic Bath: Ground-State Phase Transitions},
  author={Zhou, Nengji and Zhang, Yuyu and L{\"u}, Zhiguo and Zhao, Yang},
  journal={Annalen der Physik},
  volume={530},
  number={10},
  pages={1800120},
  year={2018},
  publisher={Wiley Online Library}
}
@article{golding1992dissipative,
  title={Dissipative quantum tunneling of a single microscopic defect in a mesoscopic metal},
  author={Golding, Brage and Zimmerman, M Neil and Coppersmith, SN},
  journal={Physical review letters},
  volume={68},
  number={7},
  pages={998},
  year={1992},
  publisher={APS}
}
@article{vojta2001kondo,
  title={Kondo effect of impurity moments in d-wave superconductors: Quantum phase transition and spectral properties},
  author={Vojta, Matthias and Bulla, Ralf},
  journal={Physical Review B},
  volume={65},
  number={1},
  pages={014511},
  year={2001},
  publisher={APS}
}
@misc{wen2004quantum,
  title={Quantum Field Theory of Many-Body Systems, Oxford Graduate Texts},
  author={Wen, XG},
  year={2004},
  publisher={Oxford University Press Oxford}
}
@article{le2018driven,
  title={Driven dissipative dynamics and topology of quantum impurity systems},
  author={Le Hur, Karyn and Henriet, Lo{\"\i}c and Herviou, Lo{\"\i}c and Plekhanov, Kirill and Petrescu, Alexandru and Goren, Tal and Schiro, Marco and Mora, Christophe and Orth, Peter P},
  journal={Comptes Rendus Physique},
  volume={19},
  number={6},
  pages={451--483},
  year={2018},
  publisher={Elsevier}
}
@article{milovsevic2010ginzburg,
  title={The Ginzburg--Landau theory in application},
  author={Milo{\v{s}}evi{\'c}, MV and Geurts, R},
  journal={Physica C: Superconductivity},
  volume={470},
  number={19},
  pages={791--795},
  year={2010},
  publisher={Elsevier}
}
@article{reed2012realization,
  title={Realization of three-qubit quantum error correction with superconducting circuits},
  author={Reed, Matthew D and DiCarlo, Leonardo and Nigg, Simon E and Sun, Luyan and Frunzio, Luigi and Girvin, Steven M and Schoelkopf, Robert J},
  journal={Nature},
  volume={482},
  number={7385},
  pages={382--385},
  year={2012},
  publisher={Nature Publishing Group}
}
@article{georgescu2020trapped,
  title={Trapped ion quantum computing turns 25},
  author={Georgescu, Iulia},
  journal={Nature Reviews Physics},
  volume={2},
  number={6},
  pages={278--278},
  year={2020},
  publisher={Nature Publishing Group}
}
@article{pastawski2011quantum,
  title={Quantum memories based on engineered dissipation},
  author={Pastawski, Fernando and Clemente, Lucas and Cirac, Juan Ignacio},
  journal={Physical Review A},
  volume={83},
  number={1},
  pages={012304},
  year={2011},
  publisher={APS}
}
@article{stock1997semiclassical,
  title={Semiclassical description of nonadiabatic quantum dynamics},
  author={Stock, Gerhard and Thoss, Michael},
  journal={Physical review letters},
  volume={78},
  number={4},
  pages={578},
  year={1997},
  publisher={APS}
}
@article{liu2021unified,
  title={Unified formulation of phase space mapping approaches for nonadiabatic quantum dynamics},
  author={Liu, Jian and He, Xin and Wu, Baihua},
  journal={Accounts of chemical research},
  volume={54},
  number={23},
  pages={4215--4228},
  year={2021},
  publisher={ACS Publications}
}
@article{runeson2019spin,
  title={Spin-mapping approach for nonadiabatic molecular dynamics},
  author={Runeson, Johan E and Richardson, Jeremy O},
  journal={The Journal of Chemical Physics},
  volume={151},
  number={4},
  pages={044119},
  year={2019},
  publisher={AIP Publishing LLC}
}
@article{barbatti2011nonadiabatic,
  title={Nonadiabatic dynamics with trajectory surface hopping method},
  author={Barbatti, Mario},
  journal={Wiley Interdisciplinary Reviews: Computational Molecular Science},
  volume={1},
  number={4},
  pages={620--633},
  year={2011},
  publisher={Wiley Online Library}
}
@article{yan2004hierarchical,
  title={Hierarchical approach based on stochastic decoupling to dissipative systems},
  author={Yan, Yun-an and Yang, Fan and Liu, Yu and Shao, Jiushu},
  journal={Chemical physics letters},
  volume={395},
  number={4-6},
  pages={216--221},
  year={2004},
  publisher={Elsevier}
}
@article{tanimura2006stochastic,
  title={Stochastic Liouville, Langevin, Fokker--Planck, and master equation approaches to quantum dissipative systems},
  author={Tanimura, Yoshitaka},
  journal={Journal of the Physical Society of Japan},
  volume={75},
  number={8},
  pages={082001},
  year={2006},
  publisher={The Physical Society of Japan}
}
@article{jin2008exact,
  title={Exact dynamics of dissipative electronic systems and quantum transport: Hierarchical equations of motion approach},
  author={Jin, Jinshuang and Zheng, Xiao and Yan, YiJing},
  journal={The Journal of chemical physics},
  volume={128},
  number={23},
  pages={234703},
  year={2008},
  publisher={American Institute of Physics}
}
@article{han2018exact,
  title={On the exact truncation tier of fermionic hierarchical equations of motion},
  author={Han, Lu and Zhang, Hou-Dao and Zheng, Xiao and Yan, YiJing},
  journal={The Journal of chemical physics},
  volume={148},
  number={23},
  pages={234108},
  year={2018},
  publisher={AIP Publishing LLC}
}
@article{zhang2020hierarchical,
  title={Hierarchical equations of motion method based on Fano spectrum decomposition for low temperature environments},
  author={Zhang, Hou-Dao and Cui, Lei and Gong, Hong and Xu, Rui-Xue and Zheng, Xiao and Yan, YiJing},
  journal={The Journal of chemical physics},
  volume={152},
  number={6},
  pages={064107},
  year={2020},
  publisher={AIP Publishing LLC}
}
@article{cui2019highly,
  title={Highly efficient and accurate sum-over-poles expansion of Fermi and Bose functions at near zero temperatures: Fano spectrum decomposition scheme},
  author={Cui, Lei and Zhang, Hou-Dao and Zheng, Xiao and Xu, Rui-Xue and Yan, YiJing},
  journal={The Journal of chemical physics},
  volume={151},
  number={2},
  pages={024110},
  year={2019},
  publisher={AIP Publishing LLC}
}
@article{gong2018quantum,
  title={Quantum entanglement of parallel-coupled double quantum dots: A theoretical study using the hierarchical equations of motion approach},
  author={Gong, Hong and Ullah, Arif and Ye, LvZhou and Zheng, Xiao and Yan, YiJing},
  journal={Chinese Journal of Chemical Physics},
  volume={31},
  number={4},
  pages={510},
  year={2018},
  publisher={Chinese Physical Society CPS}
}
@misc{hu2010communication,
  title={Communication: Pad{\'e} spectrum decomposition of Fermi function and Bose function},
  author={Hu, Jie and Xu, Rui-Xue and Yan, Yijing},
  year={2010},
  publisher={American Institute of Physics}
}
@article{shi2009efficient,
  title={Efficient hierarchical Liouville space propagator to quantum dissipative dynamics},
  author={Shi, Qiang and Chen, Liping and Nan, Guangjun and Xu, Rui-Xue and Yan, YiJing},
  journal={The Journal of chemical physics},
  volume={130},
  number={8},
  pages={084105},
  year={2009},
  publisher={American Institute of Physics}
}
@article{tanimura1989time,
  title={Time evolution of a quantum system in contact with a nearly Gaussian-Markoffian noise bath},
  author={Tanimura, Yoshitaka and Kubo, Ryogo},
  journal={Journal of the Physical Society of Japan},
  volume={58},
  number={1},
  pages={101--114},
  year={1989},
  publisher={The Physical Society of Japan}
}
@article{liu2014reduced,
  title={Reduced quantum dynamics with arbitrary bath spectral densities: Hierarchical equations of motion based on several different bath decomposition schemes},
  author={Liu, Hao and Zhu, Lili and Bai, Shuming and Shi, Qiang},
  journal={The Journal of chemical physics},
  volume={140},
  number={13},
  pages={134106},
  year={2014},
  publisher={American Institute of Physics}
}
@article{stockburger2002exact,
  title={Exact c-number representation of non-Markovian quantum dissipation},
  author={Stockburger, J{\"u}rgen T and Grabert, Hermann},
  journal={Physical review letters},
  volume={88},
  number={17},
  pages={170407},
  year={2002},
  publisher={APS}
}
@article{koch2008non,
  title={Non-Markovian dissipative semiclassical dynamics},
  author={Koch, Werner and Gro{\ss}mann, Frank and Stockburger, J{\"u}rgen T and Ankerhold, Joachim},
  journal={Physical review letters},
  volume={100},
  number={23},
  pages={230402},
  year={2008},
  publisher={APS}
}
@article{stockburger2016exact,
  title={Exact propagation of open quantum systems in a system-reservoir context},
  author={Stockburger, J{\"u}rgen T},
  journal={EPL (Europhysics Letters)},
  volume={115},
  number={4},
  pages={40010},
  year={2016},
  publisher={IOP Publishing}
}
@article{schmitz2019variance,
  title={A variance reduction technique for the stochastic Liouville--von Neumann equation},
  author={Schmitz, Konstantin and Stockburger, J{\"u}rgen T},
  journal={The European Physical Journal Special Topics},
  volume={227},
  number={15},
  pages={1929--1937},
  year={2019},
  publisher={Springer}
}
@article{shao2004decoupling,
  title={Decoupling quantum dissipation interaction via stochastic fields},
  author={Shao, Jiushu},
  journal={The Journal of chemical physics},
  volume={120},
  number={11},
  pages={5053--5056},
  year={2004},
  publisher={American Institute of Physics}
}
@article{shao2010rigorous,
  title={Rigorous representation and exact simulation of real Gaussian stationary processes},
  author={Shao, Jiushu},
  journal={Chemical Physics},
  volume={375},
  number={2-3},
  pages={378--379},
  year={2010},
  publisher={Elsevier}
}
@article{hsieh2018unified,
  title={A unified stochastic formulation of dissipative quantum dynamics. II. Beyond linear response of spin baths},
  author={Hsieh, Chang-Yu and Cao, Jianshu},
  journal={The Journal of chemical physics},
  volume={148},
  number={1},
  pages={014104},
  year={2018},
  publisher={AIP Publishing LLC}
}
@article{mccaul2017partition,
  title={Partition-free approach to open quantum systems in harmonic environments: An exact stochastic Liouville equation},
  author={McCaul, GMG and Lorenz, CD and Kantorovich, L},
  journal={Physical Review B},
  volume={95},
  number={12},
  pages={125124},
  year={2017},
  publisher={APS}
}
@article{ke2016hierarchy,
  title={Hierarchy of forward-backward stochastic Schr{\"o}dinger equation},
  author={Ke, Yaling and Zhao, Yi},
  journal={The Journal of chemical physics},
  volume={145},
  number={2},
  pages={024101},
  year={2016},
  publisher={AIP Publishing LLC}
}
@article{ke2017extension,
  title={An extension of stochastic hierarchy equations of motion for the equilibrium correlation functions},
  author={Ke, Yaling and Zhao, Yi},
  journal={The Journal of chemical physics},
  volume={146},
  number={21},
  pages={214105},
  year={2017},
  publisher={AIP Publishing LLC}
}
@article{han2019stochastic,
  title={Stochastic Representation of Non-Markovian Fermionic Quantum Dissipation},
  author={Han, Lu and Chernyak, Vladimir and Yan, Yun-An and Zheng, Xiao and Yan, YiJing},
  journal={Physical review letters},
  volume={123},
  number={5},
  pages={050601},
  year={2019},
  publisher={APS}
}
@article{xu2015dissipaton,
  title={Dissipaton equation of motion for system-and-bath interference dynamics},
  author={Xu, Rui-Xue and Zhang, Hou-Dao and Zheng, Xiao and Yan, Yijing},
  journal={Science China Chemistry},
  volume={58},
  pages={1816--1824},
  year={2015},
  publisher={Springer}
}
@article{yan2022piecewise,
  title={Piecewise ensemble averaging stochastic Liouville equations for simulating non-Markovian quantum dynamics},
  author={Yan, Yun-An and Zheng, Xiao and Shao, Jiushu},
  journal={New Journal of Physics},
  volume={24},
  number={10},
  pages={103012},
  year={2022},
  publisher={IOP Publishing}
}
@article{chen2022universal,
  title={Universal time-domain Prony fitting decomposition for optimized hierarchical quantum master equations},
  author={Chen, Zi-Hao and Wang, Yao and Zheng, Xiao and Xu, Rui-Xue and Yan, YiJing},
  journal={The Journal of Chemical Physics},
  volume={156},
  pages={221102},
  year={2022},
  publisher={AIP Publishing LLC}
}
@article{shao2022dynamics,
  title={Dynamics of the spin-boson model at zero temperature and strong dissipation},
  author={Shao, Jiushu},
  journal={Physical Review A},
  volume={105},
  number={5},
  pages={052201},
  year={2022},
  publisher={APS}
}
@article{moix2013hybrid,
  title={A hybrid stochastic hierarchy equations of motion approach to treat the low temperature dynamics of non-Markovian open quantum systems},
  author={Moix, Jeremy M and Cao, Jianshu},
  journal={The Journal of chemical physics},
  volume={139},
  number={13},
  pages={134106},
  year={2013},
  publisher={American Institute of Physics}
}
@article{ying2023spin,
  title={Spin relaxation dynamics with a continuous spin environment: the dissipaton equation of motion approach},
  author={Ying, Wenxiang and Su, Yu and Chen, Zi-Hao and Wang, Yao and Huo, Pengfei},
  journal={arXiv preprint arXiv:2302.00215},
  year={2023}
}
@article{luchnikov2022probing,
  title={Probing non-Markovian quantum dynamics with data-driven analysis: Beyond “black-box” machine-learning models},
  author={Luchnikov, IA and Kiktenko, EO and Gavreev, MA and Ouerdane, H and Filippov, SN and Fedorov, AK},
  journal={Physical Review Research},
  volume={4},
  number={4},
  pages={043002},
  year={2022},
  publisher={APS}
}
@article{tang2022fewest,
  title={Fewest-Switches Surface Hopping with Long Short-Term Memory Networks},
  author={Tang, Diandong and Jia, Luyang and Shen, Lin and Fang, Wei-Hai},
  journal={The Journal of Physical Chemistry Letters},
  volume={13},
  number={44},
  pages={10377--10387},
  year={2022},
  publisher={ACS Publications}
}
@article{yao2022emulating,
  title={Emulating Quantum Dynamics with Neural Networks via Knowledge Distillation},
  author={Yao, Yu and Cao, Chao and Haas, Stephan and Agarwal, Mahak and Khanna, Divyam and Abram, Marcin},
  journal={arXiv preprint arXiv:2203.10200},
  year={2022}
}
@article{naicker2022machine,
  title={Machine learning for excitation energy transfer dynamics},
  author={Naicker, Kimara and Sinayskiy, Ilya and Petruccione, Francesco},
  journal={Physical Review Research},
  volume={4},
  number={3},
  pages={033175},
  year={2022},
  publisher={APS}
}
@article{kadupitiya2022solving,
  title={Solving Newton’s equations of motion with large timesteps using recurrent neural networks based operators},
  author={Kadupitiya, JCS and Fox, Geoffrey C and Jadhao, Vikram},
  journal={Machine Learning: Science and Technology},
  volume={3},
  number={2},
  pages={025002},
  year={2022},
  publisher={IOP Publishing}
}
@article{choi2022learning,
  title={Learning quantum dynamics with latent neural ordinary differential equations},
  author={Choi, Matthew and Flam-Shepherd, Daniel and Kyaw, Thi Ha and Aspuru-Guzik, Al{\'a}n},
  journal={Physical Review A},
  volume={105},
  number={4},
  pages={042403},
  year={2022},
  publisher={APS}
}
@article{yang2020applications,
  title={Applications of neural networks to dynamics simulation of Landau-Zener transitions},
  author={Yang, Bianjiang and He, Baizhe and Wan, Jiajun and Kubal, Sharvaj and Zhao, Yang},
  journal={Chemical Physics},
  volume={528},
  pages={110509},
  year={2020},
  publisher={Elsevier}
}

@article{bandyopadhyay2018applications,
  title={Applications of neural networks to the simulation of dynamics of open quantum systems},
  author={Bandyopadhyay, Sayantan and Huang, Zhongkai and Sun, Kewei and Zhao, Yang},
  journal={Chemical Physics},
  volume={515},
  pages={272--278},
  year={2018},
  publisher={Elsevier}
}
@article{secor2021artificial,
  title={Artificial neural networks as propagators in quantum dynamics},
  author={Secor, Maxim and Soudackov, Alexander V and Hammes-Schiffer, Sharon},
  journal={The Journal of Physical Chemistry Letters},
  volume={12},
  number={43},
  pages={10654--10662},
  year={2021},
  publisher={ACS Publications}
}
@article{hase2016machine,
  title={Machine learning exciton dynamics},
  author={H{\"a}se, Florian and Valleau, St{\'e}phanie and Pyzer-Knapp, Edward and Aspuru-Guzik, Al{\'a}n},
  journal={Chemical Science},
  volume={7},
  number={8},
  pages={5139--5147},
  year={2016},
  publisher={Royal Society of Chemistry}
}
@article{hase2017machine,
  title={Machine learning for quantum dynamics: deep learning of excitation energy transfer properties},
  author={H{\"a}se, Florian and Kreisbeck, Christoph and Aspuru-Guzik, Al{\'a}n},
  journal={Chemical science},
  volume={8},
  number={12},
  pages={8419--8426},
  year={2017},
  publisher={Royal Society of Chemistry}
}
@article{ge2022four,
  title={Four-dimensional spacetime atomistic artificial intelligence models},
  author={Ge, Fuchun and Zhang, Lina and Ullah, Arif and Dral, Pavlo O},
  journal={ChemRxiv},
  year={2022}
}
@article{hartmann2019neural,
  title={Neural-network approach to dissipative quantum many-body dynamics},
  author={Hartmann, Michael J and Carleo, Giuseppe},
  journal={Physical review letters},
  volume={122},
  number={25},
  pages={250502},
  year={2019},
  publisher={APS}
}
@article{wang2021spacetime,
  title={Spacetime neural network for high dimensional quantum dynamics},
  author={Wang, Jiangran and Chen, Zhuo and Luo, Di and Zhao, Zhizhen and Hur, Vera Mikyoung and Clark, Bryan K},
  journal={arXiv preprint arXiv:2108.02200},
  year={2021}
}
@article{akimov2021extending,
  title={Extending the time scales of nonadiabatic molecular dynamics via machine learning in the time domain},
  author={Akimov, Alexey V},
  journal={The Journal of Physical Chemistry Letters},
  volume={12},
  number={50},
  pages={12119--12128},
  year={2021},
  publisher={ACS Publications}
}
@article{farahvash2020machine,
  title={Machine learning Frenkel Hamiltonian parameters to accelerate simulations of exciton dynamics},
  author={Farahvash, Ardavan and Lee, Chee-Kong and Sun, Qiming and Shi, Liang and Willard, Adam P},
  journal={The Journal of Chemical Physics},
  volume={153},
  number={7},
  pages={074111},
  year={2020},
  publisher={AIP Publishing LLC}
}
@article{wu2021forecasting,
  title={Forecasting nonadiabatic dynamics using hybrid convolutional neural network/long short-term memory network},
  author={Wu, Daxin and Hu, Zhubin and Li, Jiebo and Sun, Xiang},
  journal={The Journal of Chemical Physics},
  volume={155},
  number={22},
  pages={224104},
  year={2021},
  publisher={AIP Publishing LLC}
}
@article{banchi2018modelling,
  title={Modelling non-markovian quantum processes with recurrent neural networks},
  author={Banchi, Leonardo and Grant, Edward and Rocchetto, Andrea and Severini, Simone},
  journal={New Journal of Physics},
  volume={20},
  number={12},
  pages={123030},
  year={2018},
  publisher={IOP Publishing}
}
@incollection{zhang2023excited,
  title={Excited-state dynamics with machine learning},
  author={Zhang, Lina and Ullah, Arif and Pinheiro Jr, Max and Dral, Pavlo O and Barbatti, Mario},
  booktitle={Quantum Chemistry in the Age of Machine Learning},
  pages={329--353},
  year={2023},
  publisher={Elsevier}
}
@article{Bergstra2015HyperoptAP,
  title={Hyperopt: a Python library for model selection and hyperparameter optimization},
  author={James Bergstra and Brent Komer and Chris Eliasmith and Daniel L. K. Yamins and David D. Cox},
  journal={Computational Science \& Discovery},
  year={2015},
  volume={8},
  pages={014008}
}
@article{bergstra2011algorithms,
  title={Algorithms for hyper-parameter optimization},
  author={Bergstra, James and Bardenet, R{\'e}mi and Bengio, Yoshua and K{\'e}gl, Bal{\'a}zs},
  journal={Advances in neural information processing systems},
  volume={24},
  year={2011}
}
@Manual{xacs2022,
  Title                    = {\textit{XACS}: Xiamen Atomistic Computing Suite. \url{http://XACScloud.com} (accessed on Feb 16, 2023)},
  Address                  = {Xiamen, China},
  Author                   = {Xiamen University},
  Organization             = {Xiamen University},
  Year                     = {2022--2023},
  HowPublished             = {Xiamen University, Xiamen, China},
  Institution              = {Xiamen University},
  Publisher                = {Xiamen University}
}
@article{von2020introducing,
  title={Introducing machine learning: science and technology},
  author={von Lilienfeld, O Anatole},
  journal={Machine Learning: Science and Technology},
  volume={1},
  number={1},
  pages={010201},
  year={2020},
  publisher={IOP Publishing}
}

@article{hornik89,
  author = {Hornik, Kurt and Stinchcombe, Maxwell and White, Halbert},
  title = {{Multilayer feedforward networks are universal approximators}},
  journal = {Neural Netw.},
  year = {1989},
  volume = {2},
  number = {5},
  pages = {359--366},
  month = jan
}

@article{cybenko89,
  author = {Cybenko, G},
  title = {{Approximation by superpositions of a sigmoidal function}},
  journal = {Math. Control Signals Syst.},
  year = {1989},
  volume = {2},
  number = {4},
  pages = {303--314},
  month = dec
}

@article{leshno93,
title = {Multilayer feedforward networks with a nonpolynomial activation function can approximate any function},
journal = {Neural Netw.},
volume = {6},
number = {6},
pages = {861-867},
year = {1993},
author = {Moshe Leshno and Vladimir Ya. Lin and Allan Pinkus and Shimon Schocken}
}
@article{mohseni2008environment,
  title={Environment-assisted quantum walks in photosynthetic energy transfer},
  author={Mohseni, Masoud and Rebentrost, Patrick and Lloyd, Seth and Aspuru-Guzik, Alan},
  journal={{J. Chem. Phys.}},
  volume={129},
  number={17},
  pages={11B603},
  year={2008},
  publisher={American Institute of Physics}
}

